Adjoint 2D QCD and Pure 3D QCD: A Comparison of Spectra

We briefly review the 1+1-dimensional SU(N) gauge theory minimally coupled to an adjoint scalar, based upon a dimensional reduction of 2+1-dimensional pure gauge theory, which approximates the dynamics of the transversely polarized gluon. The lightest glueball states are investigated non-perturbatively using light-front quantisation in the large-N limit a la 't Hooft, and the physical meaning of the results elucidated. Comparison is made with recent lattice Monte Carlo data for 3-dimensional quenched QCD.

==> figure2 <==
%!
%%Creator: Mathematica
%%AspectRatio: .61803 
MathPictureStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 0.142857 0 0.0772542 [
[(1)] .14286 0 0 2 Msboxa
[(2)] .28571 0 0 2 Msboxa
[(3)] .42857 0 0 2 Msboxa
[(4)] .57143 0 0 2 Msboxa
[(5)] .71429 0 0 2 Msboxa
[(6)] .85714 0 0 2 Msboxa
[(7)] 1 0 0 2 Msboxa
[(<n>)] 1.025 0 -1 0 Msboxa
[(FIGURE 2)] .5 .61803 0 -2 0 0 1 Mouter Mrotsboxa
[(0)] -0.0125 0 1 0 Msboxa
[(1)] -0.0125 .07725 1 0 Msboxa
[(2)] -0.0125 .15451 1 0 Msboxa
[(3)] -0.0125 .23176 1 0 Msboxa
[(4)] -0.0125 .30902 1 0 Msboxa
[(5)] -0.0125 .38627 1 0 Msboxa
[(6)] -0.0125 .46353 1 0 Msboxa
[(7)] -0.0125 .54078 1 0 Msboxa
[(8)] -0.0125 .61803 1 0 Msboxa
[(M)] 0 .61803 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 .61903 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
0 g
p
p
.002 w
.14286 0 m
.14286 .00625 L
s
P
[(1)] .14286 0 0 2 Mshowa
p
.002 w
.28571 0 m
.28571 .00625 L
s
P
[(2)] .28571 0 0 2 Mshowa
p
.002 w
.42857 0 m
.42857 .00625 L
s
P
[(3)] .42857 0 0 2 Mshowa
p
.002 w
.57143 0 m
.57143 .00625 L
s
P
[(4)] .57143 0 0 2 Mshowa
p
.002 w
.71429 0 m
.71429 .00625 L
s
P
[(5)] .71429 0 0 2 Mshowa
p
.002 w
.85714 0 m
.85714 .00625 L
s
P
[(6)] .85714 0 0 2 Mshowa
p
.002 w
1 0 m
1 .00625 L
s
P
[(7)] 1 0 0 2 Mshowa
p
.001 w
.02857 0 m
.02857 .00375 L
s
P
p
.001 w
.05714 0 m
.05714 .00375 L
s
P
p
.001 w
.08571 0 m
.08571 .00375 L
s
P
p
.001 w
.11429 0 m
.11429 .00375 L
s
P
p
.001 w
.17143 0 m
.17143 .00375 L
s
P
p
.001 w
.2 0 m
.2 .00375 L
s
P
p
.001 w
.22857 0 m
.22857 .00375 L
s
P
p
.001 w
.25714 0 m
.25714 .00375 L
s
P
p
.001 w
.31429 0 m
.31429 .00375 L
s
P
p
.001 w
.34286 0 m
.34286 .00375 L
s
P
p
.001 w
.37143 0 m
.37143 .00375 L
s
P
p
.001 w
.4 0 m
.4 .00375 L
s
P
p
.001 w
.45714 0 m
.45714 .00375 L
s
P
p
.001 w
.48571 0 m
.48571 .00375 L
s
P
p
.001 w
.51429 0 m
.51429 .00375 L
s
P
p
.001 w
.54286 0 m
.54286 .00375 L
s
P
p
.001 w
.6 0 m
.6 .00375 L
s
P
p
.001 w
.62857 0 m
.62857 .00375 L
s
P
p
.001 w
.65714 0 m
.65714 .00375 L
s
P
p
.001 w
.68571 0 m
.68571 .00375 L
s
P
p
.001 w
.74286 0 m
.74286 .00375 L
s
P
p
.001 w
.77143 0 m
.77143 .00375 L
s
P
p
.001 w
.8 0 m
.8 .00375 L
s
P
p
.001 w
.82857 0 m
.82857 .00375 L
s
P
p
.001 w
.88571 0 m
.88571 .00375 L
s
P
p
.001 w
.91429 0 m
.91429 .00375 L
s
P
p
.001 w
.94286 0 m
.94286 .00375 L
s
P
p
.001 w
.97143 0 m
.97143 .00375 L
s
P
[(<n>)] 1.025 0 -1 0 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(FIGURE 2)] .5 .61803 0 -2 0 0 1 Mouter Mrotshowa
p
.002 w
0 0 m
.00625 0 L
s
P
[(0)] -0.0125 0 1 0 Mshowa
p
.002 w
0 .07725 m
.00625 .07725 L
s
P
[(1)] -0.0125 .07725 1 0 Mshowa
p
.002 w
0 .15451 m
.00625 .15451 L
s
P
[(2)] -0.0125 .15451 1 0 Mshowa
p
.002 w
0 .23176 m
.00625 .23176 L
s
P
[(3)] -0.0125 .23176 1 0 Mshowa
p
.002 w
0 .30902 m
.00625 .30902 L
s
P
[(4)] -0.0125 .30902 1 0 Mshowa
p
.002 w
0 .38627 m
.00625 .38627 L
s
P
[(5)] -0.0125 .38627 1 0 Mshowa
p
.002 w
0 .46353 m
.00625 .46353 L
s
P
[(6)] -0.0125 .46353 1 0 Mshowa
p
.002 w
0 .54078 m
.00625 .54078 L
s
P
[(7)] -0.0125 .54078 1 0 Mshowa
p
.002 w
0 .61803 m
.00625 .61803 L
s
P
[(8)] -0.0125 .61803 1 0 Mshowa
p
.001 w
0 .01545 m
.00375 .01545 L
s
P
p
.001 w
0 .0309 m
.00375 .0309 L
s
P
p
.001 w
0 .04635 m
.00375 .04635 L
s
P
p
.001 w
0 .0618 m
.00375 .0618 L
s
P
p
.001 w
0 .09271 m
.00375 .09271 L
s
P
p
.001 w
0 .10816 m
.00375 .10816 L
s
P
p
.001 w
0 .12361 m
.00375 .12361 L
s
P
p
.001 w
0 .13906 m
.00375 .13906 L
s
P
p
.001 w
0 .16996 m
.00375 .16996 L
s
P
p
.001 w
0 .18541 m
.00375 .18541 L
s
P
p
.001 w
0 .20086 m
.00375 .20086 L
s
P
p
.001 w
0 .21631 m
.00375 .21631 L
s
P
p
.001 w
0 .24721 m
.00375 .24721 L
s
P
p
.001 w
0 .26266 m
.00375 .26266 L
s
P
p
.001 w
0 .27812 m
.00375 .27812 L
s
P
p
.001 w
0 .29357 m
.00375 .29357 L
s
P
p
.001 w
0 .32447 m
.00375 .32447 L
s
P
p
.001 w
0 .33992 m
.00375 .33992 L
s
P
p
.001 w
0 .35537 m
.00375 .35537 L
s
P
p
.001 w
0 .37082 m
.00375 .37082 L
s
P
p
.001 w
0 .40172 m
.00375 .40172 L
s
P
p
.001 w
0 .41717 m
.00375 .41717 L
s
P
p
.001 w
0 .43262 m
.00375 .43262 L
s
P
p
.001 w
0 .44807 m
.00375 .44807 L
s
P
p
.001 w
0 .47898 m
.00375 .47898 L
s
P
p
.001 w
0 .49443 m
.00375 .49443 L
s
P
p
.001 w
0 .50988 m
.00375 .50988 L
s
P
p
.001 w
0 .52533 m
.00375 .52533 L
s
P
p
.001 w
0 .55623 m
.00375 .55623 L
s
P
p
.001 w
0 .57168 m
.00375 .57168 L
s
P
p
.001 w
0 .58713 m
.00375 .58713 L
s
P
p
.001 w
0 .60258 m
.00375 .60258 L
s
P
[(M)] 0 .61803 0 -4 Mshowa
p
.002 w
0 0 m
0 .61803 L
s
P
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
.008 w
.28571 .16223 Mdot
.42857 .26266 Mdot
.57143 .36309 Mdot
.71429 .4558 Mdot
.31 .4867 Mdot
.44286 .50988 Mdot
.84286 .54851 Mdot
.57143 .57168 Mdot
P
p
[(\(++\))] .32857 .14678 0 0 Mshowa
[(\(+-\))] .47143 .24721 0 0 Mshowa
[(\(++\))] .61429 .34764 0 0 Mshowa
[(\(+-\))] .75714 .44035 0 0 Mshowa
[(\(++\))] .88571 .53305 0 0 Mshowa
[(\(++\))] .31429 .46353 0 0 Mshowa
[(\(--\))] .45714 .4867 0 0 Mshowa
[(\(++\)/\(-+\)?)] .61429 .54851 0 0 Mshowa
P
P
% End of Graphics
MathPictureEnd


==> figure3 <==
%!
%%Creator: Mathematica
%%AspectRatio: .61803 
MathPictureStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0.0238095 0.47619 0.0147151 0.47619 [
[(FIGURE 3)] .5 .61803 0 -2 Msboxa
[ 0 0 0 0 ]
[ 1 .61803 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
0 g
p
[(FIGURE 3)] .5 .61803 0 -2 Mshowa
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
% Start of sub-graphic
p
0.0238095 0.0147151 0.477324 0.295003 MathSubStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 1 0 0.0441453 [
[(0.2)] .2 0 0 2 Msboxa
[(0.4)] .4 0 0 2 Msboxa
[(0.6)] .6 0 0 2 Msboxa
[(0.8)] .8 0 0 2 Msboxa
[(1)] 1 0 0 2 Msboxa
[(x)] 1.025 0 -1 0 Msboxa
[(\(c\))] .5 .61803 0 -2 0 0 1 Mouter Mrotsboxa
[(0)] -0.0125 0 1 0 Msboxa
[(2)] -0.0125 .08829 1 0 Msboxa
[(4)] -0.0125 .17658 1 0 Msboxa
[(6)] -0.0125 .26487 1 0 Msboxa
[(8)] -0.0125 .35316 1 0 Msboxa
[(10)] -0.0125 .44145 1 0 Msboxa
[(12)] -0.0125 .52974 1 0 Msboxa
[(14)] -0.0125 .61803 1 0 Msboxa
[( g\(x\))] 0 .61803 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 .61903 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
p
p
.002 w
.2 0 m
.2 .00625 L
s
P
[(0.2)] .2 0 0 2 Mshowa
p
.002 w
.4 0 m
.4 .00625 L
s
P
[(0.4)] .4 0 0 2 Mshowa
p
.002 w
.6 0 m
.6 .00625 L
s
P
[(0.6)] .6 0 0 2 Mshowa
p
.002 w
.8 0 m
.8 .00625 L
s
P
[(0.8)] .8 0 0 2 Mshowa
p
.002 w
1 0 m
1 .00625 L
s
P
[(1)] 1 0 0 2 Mshowa
p
.001 w
.04 0 m
.04 .00375 L
s
P
p
.001 w
.08 0 m
.08 .00375 L
s
P
p
.001 w
.12 0 m
.12 .00375 L
s
P
p
.001 w
.16 0 m
.16 .00375 L
s
P
p
.001 w
.24 0 m
.24 .00375 L
s
P
p
.001 w
.28 0 m
.28 .00375 L
s
P
p
.001 w
.32 0 m
.32 .00375 L
s
P
p
.001 w
.36 0 m
.36 .00375 L
s
P
p
.001 w
.44 0 m
.44 .00375 L
s
P
p
.001 w
.48 0 m
.48 .00375 L
s
P
p
.001 w
.52 0 m
.52 .00375 L
s
P
p
.001 w
.56 0 m
.56 .00375 L
s
P
p
.001 w
.64 0 m
.64 .00375 L
s
P
p
.001 w
.68 0 m
.68 .00375 L
s
P
p
.001 w
.72 0 m
.72 .00375 L
s
P
p
.001 w
.76 0 m
.76 .00375 L
s
P
p
.001 w
.84 0 m
.84 .00375 L
s
P
p
.001 w
.88 0 m
.88 .00375 L
s
P
p
.001 w
.92 0 m
.92 .00375 L
s
P
p
.001 w
.96 0 m
.96 .00375 L
s
P
[(x)] 1.025 0 -1 0 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(\(c\))] .5 .61803 0 -2 0 0 1 Mouter Mrotshowa
p
.002 w
0 0 m
.00625 0 L
s
P
[(0)] -0.0125 0 1 0 Mshowa
p
.002 w
0 .08829 m
.00625 .08829 L
s
P
[(2)] -0.0125 .08829 1 0 Mshowa
p
.002 w
0 .17658 m
.00625 .17658 L
s
P
[(4)] -0.0125 .17658 1 0 Mshowa
p
.002 w
0 .26487 m
.00625 .26487 L
s
P
[(6)] -0.0125 .26487 1 0 Mshowa
p
.002 w
0 .35316 m
.00625 .35316 L
s
P
[(8)] -0.0125 .35316 1 0 Mshowa
p
.002 w
0 .44145 m
.00625 .44145 L
s
P
[(10)] -0.0125 .44145 1 0 Mshowa
p
.002 w
0 .52974 m
.00625 .52974 L
s
P
[(12)] -0.0125 .52974 1 0 Mshowa
p
.002 w
0 .61803 m
.00625 .61803 L
s
P
[(14)] -0.0125 .61803 1 0 Mshowa
p
.001 w
0 .01766 m
.00375 .01766 L
s
P
p
.001 w
0 .03532 m
.00375 .03532 L
s
P
p
.001 w
0 .05297 m
.00375 .05297 L
s
P
p
.001 w
0 .07063 m
.00375 .07063 L
s
P
p
.001 w
0 .10595 m
.00375 .10595 L
s
P
p
.001 w
0 .12361 m
.00375 .12361 L
s
P
p
.001 w
0 .14126 m
.00375 .14126 L
s
P
p
.001 w
0 .15892 m
.00375 .15892 L
s
P
p
.001 w
0 .19424 m
.00375 .19424 L
s
P
p
.001 w
0 .2119 m
.00375 .2119 L
s
P
p
.001 w
0 .22956 m
.00375 .22956 L
s
P
p
.001 w
0 .24721 m
.00375 .24721 L
s
P
p
.001 w
0 .28253 m
.00375 .28253 L
s
P
p
.001 w
0 .30019 m
.00375 .30019 L
s
P
p
.001 w
0 .31785 m
.00375 .31785 L
s
P
p
.001 w
0 .3355 m
.00375 .3355 L
s
P
p
.001 w
0 .37082 m
.00375 .37082 L
s
P
p
.001 w
0 .38848 m
.00375 .38848 L
s
P
p
.001 w
0 .40614 m
.00375 .40614 L
s
P
p
.001 w
0 .42379 m
.00375 .42379 L
s
P
p
.001 w
0 .45911 m
.00375 .45911 L
s
P
p
.001 w
0 .47677 m
.00375 .47677 L
s
P
p
.001 w
0 .49443 m
.00375 .49443 L
s
P
p
.001 w
0 .51209 m
.00375 .51209 L
s
P
p
.001 w
0 .5474 m
.00375 .5474 L
s
P
p
.001 w
0 .56506 m
.00375 .56506 L
s
P
p
.001 w
0 .58272 m
.00375 .58272 L
s
P
p
.001 w
0 .60038 m
.00375 .60038 L
s
P
[( g\(x\))] 0 .61803 0 -4 Mshowa
p
.002 w
0 0 m
0 .61803 L
s
P
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
4 Mabswid
.04167 .37083 Mdot
.04167 .60444 Mdot
.125 .41008 Mdot
.125 .49972 Mdot
.20833 .30791 Mdot
.20833 .39324 Mdot
.29167 .20788 Mdot
.29167 .33492 Mdot
.375 .13058 Mdot
.375 .25488 Mdot
.45833 .04293 Mdot
.45833 .17249 Mdot
.54167 .03409 Mdot
.54167 .10226 Mdot
.625 .0516 Mdot
.625 .10085 Mdot
.70833 .02102 Mdot
.70833 .12369 Mdot
.79167 .00625 Mdot
.79167 .06953 Mdot
.875 .00118 Mdot
.875 .01879 Mdot
.95833 .00029 Mdot
.95833 .00843 Mdot
P
p
p
.004 w
.04167 .37083 m
.06076 .38501 L
.07986 .39613 L
.08941 .40051 L
.09896 .40412 L
.10851 .40695 L
.11806 .40901 L
.12283 .40976 L
.12522 .41006 L
.1276 .41031 L
.12999 .41052 L
.13238 .41068 L
.13357 .41074 L
.13477 .4108 L
.13596 .41084 L
.13715 .41086 L
.13835 .41088 L
.13954 .41089 L
.14073 .41088 L
.14193 .41087 L
.14312 .41084 L
.14431 .4108 L
.1467 .41069 L
.14909 .41053 L
.15148 .41033 L
.15625 .40979 L
.16102 .40909 L
.1658 .40821 L
.17535 .40595 L
.1849 .40305 L
.19444 .39952 L
.23264 .37974 L
.27083 .35232 L
.30903 .31928 L
.34722 .28264 L
.38542 .24431 L
.42361 .20604 L
.46181 .1693 L
.5 .13529 L
.53819 .10487 L
.57639 .07861 L
.61458 .05674 L
.65278 .03924 L
.69097 .02584 L
.71007 .02053 L
.72917 .01607 L
.74826 .01236 L
.76736 .00933 L
.78646 .0069 L
.80556 .00499 L
Mistroke
.82465 .0035 L
.84375 .00237 L
.86285 .00154 L
.8724 .00121 L
.88194 .00094 L
.89149 .00072 L
.90104 .00054 L
.91059 .0004 L
.91536 .00034 L
.92014 .0003 L
.92491 .00026 L
.9273 .00025 L
.92969 .00024 L
.93207 .00023 L
.93327 .00022 L
.93446 .00022 L
.93566 .00022 L
.93685 .00022 L
.93804 .00022 L
.93924 .00021 L
.94043 .00021 L
.94162 .00022 L
.94282 .00022 L
.94401 .00022 L
.9452 .00022 L
.9464 .00022 L
.94878 .00023 L
.95117 .00025 L
.95356 .00026 L
.95833 .0003 L
Mfstroke
P
P
p
[ .02 .02 ] 0 setdash
p
.004 w
.04167 .60444 m
.06076 .58834 L
.07031 .58168 L
.07986 .57352 L
.08941 .56296 L
.09896 .5496 L
.11806 .51469 L
.15625 .42431 L
.19444 .33513 L
.21354 .29861 L
.23264 .26875 L
.27083 .22574 L
.30903 .19377 L
.34722 .15984 L
.38542 .11879 L
.42361 .07534 L
.44271 .05606 L
.45226 .0477 L
.46181 .04042 L
.47135 .03436 L
.47613 .03184 L
.4809 .02966 L
.48568 .02784 L
.49045 .02639 L
.49523 .02532 L
.49761 .02492 L
.49881 .02476 L
.5 .02462 L
.50119 .02451 L
.50239 .02442 L
.50358 .02435 L
.50477 .0243 L
.50597 .02428 L
.50716 .02429 L
.50835 .02431 L
.50955 .02436 L
.51074 .02444 L
.51194 .02454 L
.51432 .0248 L
.51671 .02516 L
.5191 .0256 L
.52387 .02677 L
.52865 .02828 L
.53819 .03231 L
.54774 .03756 L
.55729 .04386 L
.57639 .0589 L
.61458 .09243 L
.63368 .10724 L
.64323 .11342 L
Mistroke
.65278 .11858 L
.66233 .12257 L
.6671 .1241 L
.67187 .1253 L
.67665 .12618 L
.67904 .1265 L
.68023 .12663 L
.68142 .12673 L
.68262 .12682 L
.68381 .12688 L
.685 .12692 L
.6862 .12695 L
.68739 .12695 L
.68858 .12693 L
.68978 .12689 L
.69097 .12683 L
.69336 .12665 L
.69455 .12653 L
.69575 .12639 L
.70052 .12562 L
.70529 .12454 L
.71007 .12316 L
.71962 .11953 L
.72917 .11485 L
.76736 .08873 L
.80556 .05888 L
.82465 .04541 L
.84375 .03375 L
.86285 .02401 L
.88194 .01612 L
.89149 .01284 L
.90104 .01003 L
.91059 .00774 L
.91536 .00682 L
.92014 .00607 L
.92253 .00577 L
.92491 .00551 L
.9273 .00531 L
.92849 .00522 L
.92969 .00516 L
.93088 .0051 L
.93207 .00506 L
.93327 .00504 L
.93446 .00503 L
.93566 .00503 L
.93685 .00505 L
.93804 .00509 L
.93924 .00515 L
.94162 .0053 L
.94282 .00541 L
Mistroke
.94401 .00553 L
.9464 .00583 L
.94878 .0062 L
.95356 .00716 L
.95833 .00843 L
Mfstroke
P
P
P
MathSubEnd
P
% End of sub-graphic
% Start of sub-graphic
p
0.522676 0.0147151 0.97619 0.295003 MathSubStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 1 0 0.0280925 [
[(0.2)] .2 0 0 2 Msboxa
[(0.4)] .4 0 0 2 Msboxa
[(0.6)] .6 0 0 2 Msboxa
[(0.8)] .8 0 0 2 Msboxa
[(1)] 1 0 0 2 Msboxa
[(x)] 1.025 0 -1 0 Msboxa
[(\(d\))] .5 .61803 0 -2 0 0 1 Mouter Mrotsboxa
[(0)] -0.0125 0 1 0 Msboxa
[(5)] -0.0125 .14046 1 0 Msboxa
[(10)] -0.0125 .28092 1 0 Msboxa
[(15)] -0.0125 .42139 1 0 Msboxa
[(20)] -0.0125 .56185 1 0 Msboxa
[(g\(x\))] 0 .61803 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 .61903 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
p
p
.002 w
.2 0 m
.2 .00625 L
s
P
[(0.2)] .2 0 0 2 Mshowa
p
.002 w
.4 0 m
.4 .00625 L
s
P
[(0.4)] .4 0 0 2 Mshowa
p
.002 w
.6 0 m
.6 .00625 L
s
P
[(0.6)] .6 0 0 2 Mshowa
p
.002 w
.8 0 m
.8 .00625 L
s
P
[(0.8)] .8 0 0 2 Mshowa
p
.002 w
1 0 m
1 .00625 L
s
P
[(1)] 1 0 0 2 Mshowa
p
.001 w
.04 0 m
.04 .00375 L
s
P
p
.001 w
.08 0 m
.08 .00375 L
s
P
p
.001 w
.12 0 m
.12 .00375 L
s
P
p
.001 w
.16 0 m
.16 .00375 L
s
P
p
.001 w
.24 0 m
.24 .00375 L
s
P
p
.001 w
.28 0 m
.28 .00375 L
s
P
p
.001 w
.32 0 m
.32 .00375 L
s
P
p
.001 w
.36 0 m
.36 .00375 L
s
P
p
.001 w
.44 0 m
.44 .00375 L
s
P
p
.001 w
.48 0 m
.48 .00375 L
s
P
p
.001 w
.52 0 m
.52 .00375 L
s
P
p
.001 w
.56 0 m
.56 .00375 L
s
P
p
.001 w
.64 0 m
.64 .00375 L
s
P
p
.001 w
.68 0 m
.68 .00375 L
s
P
p
.001 w
.72 0 m
.72 .00375 L
s
P
p
.001 w
.76 0 m
.76 .00375 L
s
P
p
.001 w
.84 0 m
.84 .00375 L
s
P
p
.001 w
.88 0 m
.88 .00375 L
s
P
p
.001 w
.92 0 m
.92 .00375 L
s
P
p
.001 w
.96 0 m
.96 .00375 L
s
P
[(x)] 1.025 0 -1 0 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(\(d\))] .5 .61803 0 -2 0 0 1 Mouter Mrotshowa
p
.002 w
0 0 m
.00625 0 L
s
P
[(0)] -0.0125 0 1 0 Mshowa
p
.002 w
0 .14046 m
.00625 .14046 L
s
P
[(5)] -0.0125 .14046 1 0 Mshowa
p
.002 w
0 .28092 m
.00625 .28092 L
s
P
[(10)] -0.0125 .28092 1 0 Mshowa
p
.002 w
0 .42139 m
.00625 .42139 L
s
P
[(15)] -0.0125 .42139 1 0 Mshowa
p
.002 w
0 .56185 m
.00625 .56185 L
s
P
[(20)] -0.0125 .56185 1 0 Mshowa
p
.001 w
0 .02809 m
.00375 .02809 L
s
P
p
.001 w
0 .05618 m
.00375 .05618 L
s
P
p
.001 w
0 .08428 m
.00375 .08428 L
s
P
p
.001 w
0 .11237 m
.00375 .11237 L
s
P
p
.001 w
0 .16855 m
.00375 .16855 L
s
P
p
.001 w
0 .19665 m
.00375 .19665 L
s
P
p
.001 w
0 .22474 m
.00375 .22474 L
s
P
p
.001 w
0 .25283 m
.00375 .25283 L
s
P
p
.001 w
0 .30902 m
.00375 .30902 L
s
P
p
.001 w
0 .33711 m
.00375 .33711 L
s
P
p
.001 w
0 .3652 m
.00375 .3652 L
s
P
p
.001 w
0 .39329 m
.00375 .39329 L
s
P
p
.001 w
0 .44948 m
.00375 .44948 L
s
P
p
.001 w
0 .47757 m
.00375 .47757 L
s
P
p
.001 w
0 .50566 m
.00375 .50566 L
s
P
p
.001 w
0 .53376 m
.00375 .53376 L
s
P
p
.001 w
0 .58994 m
.00375 .58994 L
s
P
[(g\(x\))] 0 .61803 0 -4 Mshowa
p
.002 w
0 0 m
0 .61803 L
s
P
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
4 Mabswid
.04167 .23598 Mdot
.04167 .5601 Mdot
.125 .26096 Mdot
.125 .55925 Mdot
.20833 .25024 Mdot
.20833 .42311 Mdot
.29167 .21313 Mdot
.29167 .25395 Mdot
.375 .12027 Mdot
.375 .1622 Mdot
.45833 .0433 Mdot
.45833 .10976 Mdot
.54167 .01253 Mdot
.54167 .06507 Mdot
.625 .00576 Mdot
.625 .03284 Mdot
.70833 .00466 Mdot
.70833 .01337 Mdot
.79167 .00254 Mdot
.79167 .00398 Mdot
.875 .00075 Mdot
.875 .00075 Mdot
.95833 .00018 Mdot
.95833 .00036 Mdot
P
p
p
.004 w
.05263 .24148 m
.07237 .24967 L
.08224 .25295 L
.09211 .25568 L
.10197 .25788 L
.10691 .25878 L
.11184 .25955 L
.11678 .26018 L
.12171 .26069 L
.12418 .2609 L
.12664 .26107 L
.12911 .26121 L
.13158 .26132 L
.13405 .2614 L
.13528 .26143 L
.13651 .26145 L
.13775 .26146 L
.13898 .26147 L
.14021 .26147 L
.14145 .26146 L
.14268 .26144 L
.14391 .26141 L
.14515 .26138 L
.14638 .26134 L
.14885 .26123 L
.15132 .2611 L
.15625 .26074 L
.16118 .26027 L
.17105 .25898 L
.18092 .25724 L
.19079 .25508 L
.21053 .24956 L
.25 .23423 L
.28947 .21434 L
.32895 .19127 L
.36842 .16642 L
.40789 .14108 L
.44737 .11638 L
.48684 .09327 L
.52632 .07244 L
.56579 .05437 L
.60526 .03926 L
.64474 .02714 L
.68421 .01782 L
.70395 .01412 L
.72368 .011 L
.74342 .00841 L
.76316 .0063 L
.78289 .00461 L
.80263 .00328 L
Mistroke
.82237 .00227 L
.84211 .00153 L
.85197 .00124 L
.86184 .001 L
.87171 .00081 L
.88158 .00065 L
.89145 .00053 L
.90132 .00044 L
.91118 .00037 L
.92105 .00031 L
.93092 .00027 L
.94079 .00024 L
.95066 .00021 L
.96053 .00018 L
.97039 .00013 L
.98026 6e-05 L
Mfstroke
.98718 0 m
.98026 6e-05 L
s
s
s
P
P
p
[ .02 .02 ] 0 setdash
p
.004 w
.05263 .57075 m
.05757 .57442 L
.0625 .57741 L
.06497 .57864 L
.06743 .57971 L
.0699 .5806 L
.07237 .58132 L
.0736 .58161 L
.07484 .58187 L
.07607 .58208 L
.0773 .58225 L
.07854 .58238 L
.07977 .58247 L
.081 .58251 L
.08224 .58252 L
.08347 .58248 L
.0847 .5824 L
.08594 .58229 L
.08717 .58213 L
.08964 .5817 L
.09211 .5811 L
.09704 .57946 L
.10197 .5772 L
.11184 .57095 L
.12171 .56251 L
.13158 .55207 L
.17105 .49394 L
.21053 .41867 L
.25 .33718 L
.28947 .25814 L
.32895 .18753 L
.36842 .12879 L
.40789 .08321 L
.42763 .06527 L
.44737 .05035 L
.46711 .03823 L
.48684 .02862 L
.50658 .02123 L
.52632 .01572 L
.53618 .01358 L
.54605 .01179 L
.55592 .01031 L
.56579 .0091 L
.57566 .00814 L
.58553 .00737 L
.59539 .00678 L
.60526 .00634 L
.61513 .006 L
.625 .00575 L
.63487 .00557 L
Mistroke
.64474 .00543 L
.66447 .00522 L
.68421 .00501 L
.70395 .00473 L
.72368 .00436 L
.76316 .00336 L
.80263 .00224 L
.82237 .00173 L
.84211 .0013 L
.86184 .00095 L
.88158 .00066 L
.90132 .00042 L
.91118 .00031 L
.91612 .00027 L
.92105 .00023 L
.92599 .0002 L
.92845 .00018 L
.93092 .00017 L
.93215 .00017 L
.93339 .00017 L
.93462 .00016 L
.93586 .00016 L
.93709 .00016 L
.93832 .00016 L
.93956 .00016 L
.94079 .00016 L
.94202 .00017 L
.94326 .00017 L
.94449 .00018 L
.94572 .00019 L
.94819 .00021 L
.95066 .00023 L
.95313 .00027 L
.95559 .00031 L
.96053 .00042 L
.96546 .00058 L
.97039 .00079 L
.97533 .00106 L
.98026 .00142 L
.9852 .00186 L
.99013 .00242 L
1 .00394 L
Mfstroke
P
P
P
MathSubEnd
P
% End of sub-graphic
P
p
% Start of sub-graphic
p
0.0238095 0.323031 0.477324 0.603319 MathSubStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 1 0 0.123607 [
[(0.2)] .2 0 0 2 Msboxa
[(0.4)] .4 0 0 2 Msboxa
[(0.6)] .6 0 0 2 Msboxa
[(0.8)] .8 0 0 2 Msboxa
[(1)] 1 0 0 2 Msboxa
[(x)] 1.025 0 -1 0 Msboxa
[(\(a\))] .5 .61803 0 -2 0 0 1 Mouter Mrotsboxa
[(0)] -0.0125 0 1 0 Msboxa
[(1)] -0.0125 .12361 1 0 Msboxa
[(2)] -0.0125 .24721 1 0 Msboxa
[(3)] -0.0125 .37082 1 0 Msboxa
[(4)] -0.0125 .49443 1 0 Msboxa
[(5)] -0.0125 .61803 1 0 Msboxa
[(g\(x\))] 0 .61803 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 .61903 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
p
p
.002 w
.2 0 m
.2 .00625 L
s
P
[(0.2)] .2 0 0 2 Mshowa
p
.002 w
.4 0 m
.4 .00625 L
s
P
[(0.4)] .4 0 0 2 Mshowa
p
.002 w
.6 0 m
.6 .00625 L
s
P
[(0.6)] .6 0 0 2 Mshowa
p
.002 w
.8 0 m
.8 .00625 L
s
P
[(0.8)] .8 0 0 2 Mshowa
p
.002 w
1 0 m
1 .00625 L
s
P
[(1)] 1 0 0 2 Mshowa
p
.001 w
.04 0 m
.04 .00375 L
s
P
p
.001 w
.08 0 m
.08 .00375 L
s
P
p
.001 w
.12 0 m
.12 .00375 L
s
P
p
.001 w
.16 0 m
.16 .00375 L
s
P
p
.001 w
.24 0 m
.24 .00375 L
s
P
p
.001 w
.28 0 m
.28 .00375 L
s
P
p
.001 w
.32 0 m
.32 .00375 L
s
P
p
.001 w
.36 0 m
.36 .00375 L
s
P
p
.001 w
.44 0 m
.44 .00375 L
s
P
p
.001 w
.48 0 m
.48 .00375 L
s
P
p
.001 w
.52 0 m
.52 .00375 L
s
P
p
.001 w
.56 0 m
.56 .00375 L
s
P
p
.001 w
.64 0 m
.64 .00375 L
s
P
p
.001 w
.68 0 m
.68 .00375 L
s
P
p
.001 w
.72 0 m
.72 .00375 L
s
P
p
.001 w
.76 0 m
.76 .00375 L
s
P
p
.001 w
.84 0 m
.84 .00375 L
s
P
p
.001 w
.88 0 m
.88 .00375 L
s
P
p
.001 w
.92 0 m
.92 .00375 L
s
P
p
.001 w
.96 0 m
.96 .00375 L
s
P
[(x)] 1.025 0 -1 0 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(\(a\))] .5 .61803 0 -2 0 0 1 Mouter Mrotshowa
p
.002 w
0 0 m
.00625 0 L
s
P
[(0)] -0.0125 0 1 0 Mshowa
p
.002 w
0 .12361 m
.00625 .12361 L
s
P
[(1)] -0.0125 .12361 1 0 Mshowa
p
.002 w
0 .24721 m
.00625 .24721 L
s
P
[(2)] -0.0125 .24721 1 0 Mshowa
p
.002 w
0 .37082 m
.00625 .37082 L
s
P
[(3)] -0.0125 .37082 1 0 Mshowa
p
.002 w
0 .49443 m
.00625 .49443 L
s
P
[(4)] -0.0125 .49443 1 0 Mshowa
p
.002 w
0 .61803 m
.00625 .61803 L
s
P
[(5)] -0.0125 .61803 1 0 Mshowa
p
.001 w
0 .02472 m
.00375 .02472 L
s
P
p
.001 w
0 .04944 m
.00375 .04944 L
s
P
p
.001 w
0 .07416 m
.00375 .07416 L
s
P
p
.001 w
0 .09889 m
.00375 .09889 L
s
P
p
.001 w
0 .14833 m
.00375 .14833 L
s
P
p
.001 w
0 .17305 m
.00375 .17305 L
s
P
p
.001 w
0 .19777 m
.00375 .19777 L
s
P
p
.001 w
0 .22249 m
.00375 .22249 L
s
P
p
.001 w
0 .27193 m
.00375 .27193 L
s
P
p
.001 w
0 .29666 m
.00375 .29666 L
s
P
p
.001 w
0 .32138 m
.00375 .32138 L
s
P
p
.001 w
0 .3461 m
.00375 .3461 L
s
P
p
.001 w
0 .39554 m
.00375 .39554 L
s
P
p
.001 w
0 .42026 m
.00375 .42026 L
s
P
p
.001 w
0 .44498 m
.00375 .44498 L
s
P
p
.001 w
0 .46971 m
.00375 .46971 L
s
P
p
.001 w
0 .51915 m
.00375 .51915 L
s
P
p
.001 w
0 .54387 m
.00375 .54387 L
s
P
p
.001 w
0 .56859 m
.00375 .56859 L
s
P
p
.001 w
0 .59331 m
.00375 .59331 L
s
P
[(g\(x\))] 0 .61803 0 -4 Mshowa
p
.002 w
0 0 m
0 .61803 L
s
P
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
4 Mabswid
.04167 .20682 Mdot
.04167 .55221 Mdot
.125 .22842 Mdot
.125 .36204 Mdot
.20833 .1057 Mdot
.20833 .24674 Mdot
.29167 .05488 Mdot
.29167 .26057 Mdot
.375 .24576 Mdot
.375 .26979 Mdot
.45833 .27437 Mdot
.45833 .45562 Mdot
.54167 .2743 Mdot
.54167 .44923 Mdot
.625 .23003 Mdot
.625 .26961 Mdot
.70833 .03242 Mdot
.70833 .2603 Mdot
.79167 .06443 Mdot
.79167 .24638 Mdot
.875 .22776 Mdot
.875 .27422 Mdot
.95833 .20449 Mdot
.95833 .39129 Mdot
P
p
p
.004 w
.04167 .20678 m
.07986 .21717 L
.11806 .22687 L
.15625 .23581 L
.19444 .24391 L
.23264 .25115 L
.27083 .25746 L
.30903 .26283 L
.34722 .26723 L
.38542 .27065 L
.40451 .27199 L
.42361 .27308 L
.44271 .27392 L
.45226 .27425 L
.46181 .27452 L
.46658 .27463 L
.47135 .27472 L
.47613 .2748 L
.4809 .27487 L
.48329 .27489 L
.48568 .27491 L
.48806 .27493 L
.49045 .27495 L
.49164 .27495 L
.49284 .27496 L
.49403 .27496 L
.49523 .27496 L
.49642 .27497 L
.49761 .27497 L
.49881 .27497 L
.5 .27497 L
.50119 .27496 L
.50239 .27496 L
.50358 .27496 L
.50477 .27495 L
.50716 .27494 L
.50955 .27492 L
.51432 .27488 L
.5191 .27482 L
.52865 .27466 L
.53819 .27443 L
.55729 .2738 L
.57639 .27292 L
.61458 .27043 L
.65278 .26698 L
.69097 .26257 L
.72917 .25721 L
.76736 .25088 L
.80556 .2436 L
.84375 .23534 L
Mistroke
.88194 .22608 L
.92014 .2158 L
.95833 .20447 L
Mfstroke
P
P
p
[ .02 .02 ] 0 setdash
p
.004 w
.04167 .55221 m
.04405 .55096 L
.04644 .54934 L
.05122 .54505 L
.05599 .53946 L
.06076 .53266 L
.07986 .49505 L
.09896 .4444 L
.11806 .38501 L
.15625 .25614 L
.17535 .19448 L
.19444 .13956 L
.21354 .09458 L
.22309 .07665 L
.23264 .0621 L
.23741 .05617 L
.24219 .05115 L
.24696 .04707 L
.24935 .04538 L
.25174 .04393 L
.25412 .04272 L
.25651 .04174 L
.2577 .04135 L
.2589 .04101 L
.26009 .04073 L
.26128 .04052 L
.26248 .04036 L
.26367 .04026 L
.26487 .04023 L
.26606 .04025 L
.26725 .04033 L
.26845 .04047 L
.26964 .04068 L
.27083 .04094 L
.27322 .04164 L
.27561 .04257 L
.28038 .04515 L
.28516 .04865 L
.28993 .05306 L
.29948 .0645 L
.30903 .07928 L
.32812 .11769 L
.34722 .16566 L
.38542 .27698 L
.42361 .38444 L
.44271 .42792 L
.45226 .44578 L
.46181 .46067 L
.47135 .47232 L
.47613 .47688 L
Mistroke
.4809 .48057 L
.48329 .48208 L
.48568 .48337 L
.48806 .48443 L
.49045 .48527 L
.49164 .4856 L
.49284 .48588 L
.49403 .4861 L
.49523 .48626 L
.49642 .48636 L
.49761 .48641 L
.49881 .4864 L
.5 .48634 L
.50119 .48622 L
.50239 .48604 L
.50358 .4858 L
.50477 .48551 L
.50716 .48475 L
.50955 .48376 L
.51432 .48112 L
.5191 .47757 L
.52865 .46787 L
.53819 .45479 L
.55729 .41936 L
.57639 .37347 L
.61458 .26212 L
.65278 .14788 L
.67187 .09854 L
.69097 .05857 L
.70052 .04289 L
.71007 .0304 L
.71484 .02541 L
.71962 .02129 L
.72439 .01804 L
.72678 .01675 L
.72917 .01568 L
.73155 .01483 L
.73275 .01449 L
.73394 .01421 L
.73513 .01398 L
.73633 .01381 L
.73752 .01369 L
.73872 .01363 L
.73991 .01363 L
.7411 .01368 L
.7423 .01379 L
.74349 .01396 L
.74588 .01445 L
.74707 .01478 L
.74826 .01517 L
Mistroke
.75304 .01727 L
.75781 .02023 L
.76259 .02405 L
.76736 .02871 L
.78646 .0552 L
.80556 .09268 L
.84375 .18937 L
.88194 .29196 L
.90104 .3361 L
.91059 .3547 L
.92014 .37031 L
.92491 .37683 L
.92969 .38241 L
.93446 .38695 L
.93685 .38882 L
.93924 .39039 L
.94162 .39167 L
.94282 .3922 L
.94401 .39264 L
.9452 .39301 L
.9464 .3933 L
.94759 .3935 L
.94878 .39361 L
.94998 .39364 L
.95117 .39359 L
.95237 .39344 L
.95356 .3932 L
.95595 .39244 L
.95714 .39192 L
.95833 .39129 L
Mfstroke
P
P
P
MathSubEnd
P
% End of sub-graphic
% Start of sub-graphic
p
0.522676 0.323031 0.97619 0.603319 MathSubStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 1 0 0.0686704 [
[(0.2)] .2 0 0 2 Msboxa
[(0.4)] .4 0 0 2 Msboxa
[(0.6)] .6 0 0 2 Msboxa
[(0.8)] .8 0 0 2 Msboxa
[(1)] 1 0 0 2 Msboxa
[(x)] 1.025 0 -1 0 Msboxa
[(\(b\))] .5 .61803 0 -2 0 0 1 Mouter Mrotsboxa
[(0)] -0.0125 0 1 0 Msboxa
[(2)] -0.0125 .13734 1 0 Msboxa
[(4)] -0.0125 .27468 1 0 Msboxa
[(6)] -0.0125 .41202 1 0 Msboxa
[(8)] -0.0125 .54936 1 0 Msboxa
[( g\(x\))] 0 .61803 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 .61903 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
p
p
.002 w
.2 0 m
.2 .00625 L
s
P
[(0.2)] .2 0 0 2 Mshowa
p
.002 w
.4 0 m
.4 .00625 L
s
P
[(0.4)] .4 0 0 2 Mshowa
p
.002 w
.6 0 m
.6 .00625 L
s
P
[(0.6)] .6 0 0 2 Mshowa
p
.002 w
.8 0 m
.8 .00625 L
s
P
[(0.8)] .8 0 0 2 Mshowa
p
.002 w
1 0 m
1 .00625 L
s
P
[(1)] 1 0 0 2 Mshowa
p
.001 w
.04 0 m
.04 .00375 L
s
P
p
.001 w
.08 0 m
.08 .00375 L
s
P
p
.001 w
.12 0 m
.12 .00375 L
s
P
p
.001 w
.16 0 m
.16 .00375 L
s
P
p
.001 w
.24 0 m
.24 .00375 L
s
P
p
.001 w
.28 0 m
.28 .00375 L
s
P
p
.001 w
.32 0 m
.32 .00375 L
s
P
p
.001 w
.36 0 m
.36 .00375 L
s
P
p
.001 w
.44 0 m
.44 .00375 L
s
P
p
.001 w
.48 0 m
.48 .00375 L
s
P
p
.001 w
.52 0 m
.52 .00375 L
s
P
p
.001 w
.56 0 m
.56 .00375 L
s
P
p
.001 w
.64 0 m
.64 .00375 L
s
P
p
.001 w
.68 0 m
.68 .00375 L
s
P
p
.001 w
.72 0 m
.72 .00375 L
s
P
p
.001 w
.76 0 m
.76 .00375 L
s
P
p
.001 w
.84 0 m
.84 .00375 L
s
P
p
.001 w
.88 0 m
.88 .00375 L
s
P
p
.001 w
.92 0 m
.92 .00375 L
s
P
p
.001 w
.96 0 m
.96 .00375 L
s
P
[(x)] 1.025 0 -1 0 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(\(b\))] .5 .61803 0 -2 0 0 1 Mouter Mrotshowa
p
.002 w
0 0 m
.00625 0 L
s
P
[(0)] -0.0125 0 1 0 Mshowa
p
.002 w
0 .13734 m
.00625 .13734 L
s
P
[(2)] -0.0125 .13734 1 0 Mshowa
p
.002 w
0 .27468 m
.00625 .27468 L
s
P
[(4)] -0.0125 .27468 1 0 Mshowa
p
.002 w
0 .41202 m
.00625 .41202 L
s
P
[(6)] -0.0125 .41202 1 0 Mshowa
p
.002 w
0 .54936 m
.00625 .54936 L
s
P
[(8)] -0.0125 .54936 1 0 Mshowa
p
.001 w
0 .02747 m
.00375 .02747 L
s
P
p
.001 w
0 .05494 m
.00375 .05494 L
s
P
p
.001 w
0 .0824 m
.00375 .0824 L
s
P
p
.001 w
0 .10987 m
.00375 .10987 L
s
P
p
.001 w
0 .16481 m
.00375 .16481 L
s
P
p
.001 w
0 .19228 m
.00375 .19228 L
s
P
p
.001 w
0 .21975 m
.00375 .21975 L
s
P
p
.001 w
0 .24721 m
.00375 .24721 L
s
P
p
.001 w
0 .30215 m
.00375 .30215 L
s
P
p
.001 w
0 .32962 m
.00375 .32962 L
s
P
p
.001 w
0 .35709 m
.00375 .35709 L
s
P
p
.001 w
0 .38455 m
.00375 .38455 L
s
P
p
.001 w
0 .43949 m
.00375 .43949 L
s
P
p
.001 w
0 .46696 m
.00375 .46696 L
s
P
p
.001 w
0 .49443 m
.00375 .49443 L
s
P
p
.001 w
0 .5219 m
.00375 .5219 L
s
P
p
.001 w
0 .57683 m
.00375 .57683 L
s
P
p
.001 w
0 .6043 m
.00375 .6043 L
s
P
[( g\(x\))] 0 .61803 0 -4 Mshowa
p
.002 w
0 0 m
0 .61803 L
s
P
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
4 Mabswid
.05263 .31163 Mdot
.05263 .61066 Mdot
.1579 .34844 Mdot
.1579 .37791 Mdot
.26316 .2072 Mdot
.26316 .34669 Mdot
.36842 .22681 Mdot
.36842 .31233 Mdot
.47368 .14908 Mdot
.47368 .25498 Mdot
.57895 .01276 Mdot
.57895 .18629 Mdot
.68421 .07814 Mdot
.68421 .11804 Mdot
.78947 .06026 Mdot
.78947 .21242 Mdot
.89474 .01976 Mdot
.89474 .13781 Mdot
1 0 Mdot
P
p
p
.004 w
.05263 .31164 m
.07237 .32153 L
.09211 .33005 L
.11184 .33718 L
.13158 .34292 L
.14145 .34527 L
.15132 .34727 L
.16118 .34893 L
.17105 .35024 L
.17599 .35077 L
.18092 .35122 L
.18586 .35158 L
.18832 .35173 L
.19079 .35186 L
.19326 .35197 L
.19572 .35205 L
.19696 .35209 L
.19819 .35212 L
.19942 .35215 L
.20066 .35217 L
.20189 .35218 L
.20313 .35219 L
.20436 .3522 L
.20559 .3522 L
.20683 .35219 L
.20806 .35218 L
.20929 .35217 L
.21053 .35215 L
.21299 .35209 L
.21546 .35202 L
.22039 .35181 L
.22533 .35152 L
.23026 .35115 L
.24013 .35018 L
.25 .3489 L
.26974 .34546 L
.28947 .34087 L
.32895 .3285 L
.36842 .31231 L
.40789 .29288 L
.44737 .27081 L
.48684 .24673 L
.52632 .22129 L
.56579 .1951 L
.60526 .16879 L
.64474 .14293 L
.68421 .11807 L
.72368 .0947 L
.76316 .07325 L
.80263 .05409 L
Mistroke
.84211 .03752 L
.88158 .02374 L
.92105 .01288 L
.94079 .00856 L
.96053 .00498 L
.98026 .00213 L
Mfstroke
.99995 0 m
.98026 .00213 L
s
s
P
P
p
[ .02 .02 ] 0 setdash
p
.004 w
.05263 .61066 m
.05373 .61092 L
.05482 .61107 L
.05592 .61111 L
.05702 .61106 L
.05811 .61091 L
.05921 .61066 L
.06031 .61031 L
.0614 .60987 L
.0636 .60871 L
.06579 .60719 L
.07018 .60314 L
.07456 .59781 L
.07895 .59131 L
.08772 .57521 L
.10526 .5333 L
.12281 .48321 L
.15789 .37791 L
.17544 .33016 L
.19298 .28906 L
.21053 .25603 L
.2193 .24274 L
.22807 .23161 L
.23684 .2226 L
.24561 .21561 L
.25439 .21053 L
.25877 .20866 L
.26316 .2072 L
.26754 .20614 L
.26974 .20575 L
.27193 .20545 L
.27303 .20533 L
.27412 .20523 L
.27522 .20516 L
.27632 .2051 L
.27741 .20506 L
.27851 .20505 L
.27961 .20505 L
.2807 .20507 L
.2818 .20511 L
.28289 .20516 L
.28509 .20532 L
.28728 .20555 L
.28947 .20584 L
.29386 .20659 L
.29825 .20755 L
.31579 .2128 L
.33333 .21892 L
.34211 .22174 L
.35088 .22411 L
Mistroke
.35526 .22508 L
.35965 .22586 L
.36184 .22618 L
.36404 .22644 L
.36623 .22665 L
.36732 .22674 L
.36842 .22681 L
.36952 .22686 L
.37061 .2269 L
.37171 .22692 L
.37281 .22693 L
.3739 .22692 L
.375 .2269 L
.3761 .22686 L
.37719 .2268 L
.37939 .22664 L
.38158 .22641 L
.38377 .2261 L
.38596 .22573 L
.39035 .22476 L
.39474 .22348 L
.40351 .22001 L
.41228 .21525 L
.42105 .20922 L
.4386 .1934 L
.47368 .14908 L
.50877 .09563 L
.52632 .06939 L
.54386 .04576 L
.5614 .02641 L
.57018 .01879 L
.57895 .01276 L
.58333 .01038 L
.58772 .00844 L
.59211 .00695 L
.5943 .00637 L
.59649 .00592 L
.59759 .00573 L
.59868 .00558 L
.59978 .00545 L
.60088 .00536 L
.60197 .00529 L
.60307 .00526 L
.60417 .00525 L
.60526 .00527 L
.60636 .00533 L
.60746 .00541 L
.60855 .00552 L
.60965 .00567 L
.61184 .00604 L
Mistroke
.61404 .00654 L
.61842 .00789 L
.62281 .00972 L
.63158 .01478 L
.64035 .02164 L
.64912 .0302 L
.68421 .07814 L
.7193 .13658 L
.73684 .16398 L
.75439 .18701 L
.76316 .19623 L
.77193 .20364 L
.77632 .20661 L
.7807 .20907 L
.78509 .21101 L
.78728 .21178 L
.78947 .21242 L
.79167 .21293 L
.79276 .21313 L
.79386 .2133 L
.79496 .21343 L
.79605 .21353 L
.79715 .2136 L
.79825 .21364 L
.79934 .21364 L
.80044 .21361 L
.80154 .21355 L
.80263 .21345 L
.80373 .21332 L
.80482 .21316 L
.80702 .21274 L
.80921 .21219 L
.8114 .21152 L
.81579 .2098 L
.82456 .20499 L
.83333 .19851 L
.84211 .19067 L
.85965 .17238 L
.89474 .13781 L
Mfstroke
P
P
P
MathSubEnd
P
% End of sub-graphic
P
P
% End of Graphics
MathPictureEnd


==> figure4 <==
%!
%%Creator: Mathematica
%%AspectRatio: 1.55556 
MathPictureStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 0.111111 1.11022e-16 0.111111 [
[(0++)] .14778 0 0 2 Msboxa
[(2++)] .37 0 0 2 Msboxa
[(0--)] .74 0 0 2 Msboxa
[(1+-)] .88889 0 0 2 Msboxa
[(FIGURE 4)] .5 1.55556 0 -2 Msboxa
[(1 \(1\))] -0.0125 .22222 1 0 Msboxa
[(1.5 \(2.4\))] -0.0125 .77778 1 0 Msboxa
[(2 \(3.8\))] -0.0125 1.33333 1 0 Msboxa
[(M/M_0\(0++\))] 0 1.55556 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 1.55656 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
0 g
p
p
.002 w
.14778 0 m
.14778 .00625 L
s
P
[(0++)] .14778 0 0 2 Mshowa
p
.002 w
.37 0 m
.37 .00625 L
s
P
[(2++)] .37 0 0 2 Mshowa
p
.002 w
.74 0 m
.74 .00625 L
s
P
[(0--)] .74 0 0 2 Mshowa
p
.002 w
.88889 0 m
.88889 .00625 L
s
P
[(1+-)] .88889 0 0 2 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(FIGURE 4)] .5 1.55556 0 -2 Mshowa
p
.002 w
0 .22222 m
.00625 .22222 L
s
P
[(1 \(1\))] -0.0125 .22222 1 0 Mshowa
p
.002 w
0 .77778 m
.00625 .77778 L
s
P
[(1.5 \(2.4\))] -0.0125 .77778 1 0 Mshowa
p
.002 w
0 1.33333 m
.00625 1.33333 L
s
P
[(2 \(3.8\))] -0.0125 1.33333 1 0 Mshowa
[(M/M_0\(0++\))] 0 1.55556 0 -4 Mshowa
p
.002 w
0 0 m
0 1.55556 L
s
P
P
0 0 m
1 0 L
1 1.55556 L
0 1.55556 L
closepath
clip
newpath
p
p
.004 w
newpath
.11111 .83889 .01111 0 365.73 arc
s
newpath
.11111 1.36111 .01111 0 365.73 arc
s
newpath
.33333 .96111 .01111 0 365.73 arc
s
newpath
.33333 1.18889 .01111 0 365.73 arc
s
P
p
.025 w
.14778 .22222 Mdot
.14778 .77778 Mdot
.14778 1.2 Mdot
.37 .96667 Mdot
.37 1.18889 Mdot
.72222 .77778 Mdot
.72222 1.19444 Mdot
P
p
.17333 .21111 m
.17333 .23333 L
.19556 .23333 L
.19556 .21111 L
F
.17333 .71111 m
.17333 .73333 L
.19556 .73333 L
.19556 .71111 L
F
.17333 1.17222 m
.17333 1.19444 L
.19556 1.19444 L
.19556 1.17222 L
F
.39556 1.01667 m
.39556 1.03889 L
.41778 1.03889 L
.41778 1.01667 L
F
.39556 1.22778 m
.39556 1.25 L
.41778 1.25 L
.41778 1.22778 L
F
.76667 1.07222 m
.76667 1.09444 L
.78889 1.09444 L
.78889 1.07222 L
F
.87778 .46111 m
.87778 .48333 L
.9 .48333 L
.9 .46111 L
F
.87778 .94444 m
.87778 .96667 L
.9 .96667 L
.9 .94444 L
F
P
p
.004 w
.14778 .74444 m
.14778 .81111 L
s
.14778 1.14444 m
.14778 1.25556 L
s
.37 .93333 m
.37 1 L
s
.37 1.11111 m
.37 1.26667 L
s
.72222 .74444 m
.72222 .81111 L
s
.72222 1.12778 m
.72222 1.26111 L
s
P
p
[(C = +1)] .25 .11111 0 0 Mshowa
[(C = -1)] .80556 .11111 0 0 Mshowa
P
P
% End of Graphics
MathPictureEnd

